Learning Mixtures of Unknown Causal Interventions

The ability to conduct interventions plays a pivotal role in learning causal relationships among variables, thus facilitating applications across diverse scientific disciplines such as genomics, economics, and machine learning. However, in many instances within these applications, the process of generating interventional data is subject to noise: rather than data being sampled directly from the intended interventional distribution, interventions often yield data sampled from a blend of both intended and unintended interventional distributions. We consider the fundamental challenge of disentangling mixed interventional and observational data within linear Structural Equation Models (SEMs) with Gaussian additive noise without the knowledge of the true causal graph. We demonstrate that conducting interventions, whether do or soft, yields distributions with sufficient diversity and properties conducive to efficiently recovering each component within the mixture. Furthermore, we establish that the sample complexity required to disentangle mixed data inversely correlates with the extent of change induced by an intervention in the equations governing the affected variable values. As a result, the causal graph can be identified up to its interventional Markov Equivalence Class, similar to scenarios where no noise influences the generation of interventional data. We further support our theoretical findings by conducting simulations wherein we perform causal discovery from such mixed data.

==> old_stuff/app_remaining_proofs.tex <==
\section{Missing Proofs}

\subsection{Remaining proofs from \refsec{sec:proof_main}}



\subsubsection{Proof of \reflemma{lemma:non_zero_c}}
\label{appendix:proof:lemma:non_zero_c}
\abhinav{Create restatble lemma here}

Showing $\bm{u}_{i}\neq \bm{0}$: We are given that $B$ is a lower triangular matrix with non-zero diagonal entries. Also, $\bm{c}_{i}=\bm{a}_{i}-\bm{a}_{i}^{'}\neq0$ and $[\bm{c}_{i}]_{t}=0, \forall t\geq i \implies \exists t\> s.t.\> [\bm{c}_{i}]_{t}\neq 0$ and let $t^{*}$ be that last index where $\bm{c}_{i}$ is non-zero. Now lets look at the $[B^{T}\bm{c}_{i}]_{t^{*}}=\bm{c}_{t^{*}}\cdot [B^{T}]_{t^{*},t^{*}}\neq0$ since $B^{T}$ is a upper triangular matrix and $[\bm{c}_{i}]_{t^{*}}\neq 0$. 

Showing $\bm{u}_{i}^{T}\bm{e}_{i}=0$:  $B\bm{e}_{i}$ is the $i^{th}$ column of lower triangular $B$ matrix $\implies [B\bm{e}_{i}]_{t}=0, \forall t<i \implies \bm{c}_{i}^{T}B\bm{e}_i=0$ since $[\bm{c}_{i}]_{t}=0, \forall t\geq i$.

\subsubsection{Proof of \reflemma{lemma:linearity_of_vec_op}}
\label{appendix:proof:lemma:linearity_of_vec_op}





\kk{$$\geq \|A^{i}-A^{j}\|_F^{2} + \|D^{i}-D^{j}\|_F^{2} + \|\eta^{i}-\eta^{j}\|^{2}_{2}$$}

\begin{lemma}[Non-Atomic Intervention Covariance Update]
Let $S_{U_1}$ and $S_{U_2}$ be the covariance matrix corresponding to the intervention on different sets of nodes $U_1$ and $U_2$ respectively. Then we have:
\begin{equation*}
\norm{S_{U_1}-S_{U_2}}_{F}^{2} \geq 
\end{equation*}   
\end{lemma}
\begin{proof}
When we intervene on the set of node $U_1$, we have:
\begin{equation}
\begin{aligned}
    B_{U_1} &= \Big{[}I-A +\sum_{i\in U_1} \bm{e}_i\bm{c}_i^{T} \Big{]}^{-1}\\
    &= B-BE_{U_1}\Big{[} I_{U_1} + C_{U_1}BE_{U_1} \Big{]}^{-1}C_{U_1}B\\
    &= B-BE_{U_1}M_{U_1}C_{U_1}B\\
\end{aligned}
\end{equation}
using Woodbury matrix identity where $M_{U_1}= \big{(}I_{U_1} + C_{U_1}BE_{U_1}\big{)}^{-1}$, $E_{U_1}=[\bm{e}_i]_{i\in U_1}$ is a $(n\times|U_1|)$ matrix whose columns are unit vector $\bm{e}_{i}, \forall i\in U_1$; $I_{U_1}$ is a $(|U_1|\times |U_1|)$ identity matrix;  $C_{U_1}^{T} = [\bm{c}_i]_{i\in U_1}$ is a $(n\times |U_1|)$ matrix whose columns are the correction vectors of adjacency matrix $\bm{c}_i, \forall i \in U_1$ and $B=(I-A)^{-1}$ corresponding to non-intervened setting.
Also, the new covariance matrix for the exogenous noise distribution is given by:
\begin{equation}
\label{eqn:noise_covariance}
\begin{aligned}
    D_{U_1} &= D-\sum_{i\in U_1}\delta_{i}\bm{e}_i\bm{e}_i^{T}\\
    &=D-E_{U_1}\Delta_{U_1}E_{U_1}^{T}
\end{aligned}
\end{equation}
where $E_{U_1}$ is the same matrix as defined above and $\Delta_{U_1}$ is a $(|U_1|\times |U_1|)$ diagonal matrix whose diagonal entries are $\delta_{i}=\sigma_{i}-\sigma_{i}^{'}$ denoting the change in the variance of exogenous noise variable of node $i\in U_{1}$. 
Next, the covariance matrix corresponding intervention on nodes $U_1$, we have 
% \abhinav{Need to include the change in noise term deltai too}:
\abhinav{Recheck a B term was missing initially. Corrected in eq 39 and 40 but check below}
\begin{equation}
\begin{aligned}
    S_{U_1} &= \big{(}B-BE_{U_1}M_{U_1}C_{U_1}B\big{)} D_{U_1} \big{(}B-BE_{U_1}M_{U_1}C_{U_1}B\big{)}^{T}\\
    &= \big{(}B-BE_{U_1}M_{U_1}C_{U_1}B\big{)} D \big{(}B-BE_{U_1}M_{U_1}C_{U_1}B\big{)}^{T} \\
    &\quad \quad \quad \quad \quad - \big{(}B-BE_{U_1}M_{U_1}C_{U_1}B\big{)} (E_{U_1}\Delta_{U_1}E_{U_1}^{T}) \big{(}B-BE_{U_1}M_{U_1}C_{U_1}B\big{)}^{T}\\
    &=BDB^{T} - BDB^{T}C_{U_1}^{T}M^{T}_{U_1}E_{U_1}^{T}B^{T}-B E_{U_1} M_{U_1} CBDB^{T} + B E_{U_1} M_{U_1} C(BDB^{T})B^{T}C_{U_1}^{T}M_{U_1}^{T}E_{U_1}^{T}B^{T}\\
    &\quad \quad \quad \quad \quad   - \big{(}B-E_{U_1}M_{U_1}C_{U_1}B\big{)} (E_{U_1}\Delta_{U_1}E_{U_1}^{T}) \big{(}B-E_{U_1}M_{U_1}C_{U_1}B\big{)}^{T}\\
\end{aligned}
\end{equation}
Lets define $\tilde{C}_{U_1} =  M_{U_1} C_{U_1}$, which is a matrix of size $(|U_1|\times n)$ and $M_{U_1}$ is lower triangular \abhinav{explain this more here why its lower triangular}. Thus we have:
\begin{equation}
\begin{aligned}
B^{-1}(S_{U_1}-S)B^{-T} &= -DB^{T}\tilde{C}_{U_1}^{T} E_{U_1}^{T} - E_{U_1} \tilde{C}_{U_1} BD + E_{U_1}\tilde{C}_{U_1} BDB^{T} \tilde{C}_{U_1} E_{U_1}\\
& \quad \quad \quad \quad \quad - \big{(}E_{U_1}-E_{U_1}M_{U_1}C_{U_1}BE_{U_1}\big{)} \Delta_{U_1}\big{(}E_{U_1}-E_{U_1}M_{U_1}C_{U_1}BE_{U_1}\big{)}^{T} \\
\end{aligned}
\end{equation}
Next, for $k\notin U_{1}$, if we look at the $(k,k)^{\text{th}}$ entry of above matrix we get:
\begin{equation}
\label{eqn:Su1_kk}
\begin{aligned}
    \bm{e}_{k}^{T} B^{-1}(S_{U_1}-S)B^{-T} \bm{e}_{k} &= -D_{kk}\bm{e}_k^{T} B^{T} \tilde{C}_{U_1}^{T} \cancelto{0}{(\bm{E}_{U_1}^{T}\bm{e}_k)} - D_{kk} \cancelto{0}{(\bm{e}_k^{T}E_{U_1})} \tilde{C}_{U_1}B\bm{e}_k + \cancelto{0}{(\bm{e}_k^{T} E_{U_1})}\tilde{C}_{U_1} BDB^{T} \tilde{C}_{U_1} E_{U_1} \bm{e}_k\\
    &=0\\
\end{aligned}
\end{equation}
Let $\tilde{\bm{c}}^{1}_{k}$ denote the $k^{\text{th}}$ column of the matrix $\tilde{C}^{T}_{U_1}$ where $\tilde{\bm{c}}^{1}_k$ has zero entries after $k^{\text{th}}$ index since $\tilde{C}^{T}_{U_1}$ is a lower triangular matrix. 
Next, for $i\in U_1$, looking at the $i^{\text{th}}$ row of the above matrix we get:
\begin{equation}
\label{eqn:Su1_ik}
 \bm{e}_{i}^{T} B^{-1}(S_{U_1}-S)B^{-T} \bm{e}_{k} = 
    \begin{cases}
    -D_{kk} \cancelto{0}{\bm{e}_i^{T}B^{T} \tilde{\bm{c}}^{1}_{i}} - D_{kk} \cancelto{0}{(\tilde{\bm{c}}^{1}_{i})^{T} B\bm{e}_i} + (\tilde{\bm{c}}^{1}_{i})^{T}S\tilde{\bm{c}}_{i}^{1} & k=i\\
    -D_{ii}\bm{e}_i^{T}B^{T}\tilde{\bm{c}}_k^{1} - D_{kk} (\tilde{\bm{c}}^{1}_{i})^{T}B \bm{e}_k + (\tilde{\bm{c}}_i^{1})^{T}S\tilde{\bm{c}}_k^{1}  &k\in U_1 \text{ and }  k\neq i\\
    0-D_{kk} (\tilde{\bm{c}}_i^{1})^{T}B\bm{e}_k+0 & k\notin U_1\\
    \end{cases}
\end{equation}
since $E_{U_1}\bm{e}_k=0$ makes the first and third term zero in the third case above. Similarly, few can derive the following expression for the covariance matrix corresponding to intervention on nodes $U_2$ i.e $S_{U_2}$:
\begin{equation}
\begin{aligned}
B^{-1}(S_{U_2}-S)B^{-T} &= -DB^{T}\tilde{C}_{U_2}^{T} E_{U_2}^{T} - E_{U_2} \tilde{C}_{U_2} BD + E_{U_2}\tilde{C}_{U_2} BDB^{T} \tilde{C}_{U_2} E_{U_2}\\
\end{aligned}
\end{equation}
where all the terms are defined analogously for the case $S_{U_1}$. Next, similar to \refeqn{eqn:Su1_kk} for $k\notin U_2$ looking at the $(k,k)^{\text{th}}$ entry of above matrix we get:
\begin{equation}
\label{eqn:Su2_kk}
\begin{aligned}
    \bm{e}_{k}^{T} B^{-1}(S_{U_2}-S)B^{-T} \bm{e}_{k} &= -D_{kk}\bm{e}_k^{T} B^{T} \tilde{C}_{U_2}^{T} \cancelto{0}{(\bm{E}_{U_2}^{T}\bm{e}_k)} - D_{kk} \cancelto{0}{(\bm{e}_k^{T}E_{U_2})} \tilde{C}_{U_2}B\bm{e}_k + \cancelto{0}{(\bm{e}_k^{T} E_{U_2})}\tilde{C}_{U_2} BDB^{T} \tilde{C}_{U_2} E_{U_2} \bm{e}_k\\
    &=0\\
\end{aligned}
\end{equation}
and similar to \ref{eqn:Su1_ik}, for $j\in U_2$, looking at the $j^{\text{th}}$ row of the above matrix we get:
\begin{equation}
\label{eqn:Su2_ik}
 \bm{e}_{j}^{T} B^{-1}(S_{U_2}-S)B^{-T} \bm{e}_{k} = 
    \begin{cases}
    -D_{kk} \cancelto{0}{\bm{e}_j^{T}B^{T} \tilde{\bm{c}}^{2}_{j}} - D_{kk} \cancelto{0}{(\tilde{\bm{c}}^{2}_{j})^{T} B\bm{e}_j} + (\tilde{\bm{c}}^{2}_{j})^{T}S\tilde{\bm{c}}_{j}^{2} & k=j\\
    -D_{jj}\bm{e}_j^{T}B^{T}\tilde{\bm{c}}_k^{2} - D_{kk} (\tilde{\bm{c}}^{2}_{j})^{T}B \bm{e}_k + (\tilde{\bm{c}}_j^{2})^{T}S\tilde{\bm{c}}_k^{2}  &k\in U_2 \text{ and }  k\neq j\\
    0-D_{kk} (\tilde{\bm{c}}_j^{2})^{T}B\bm{e}_k+0 & k\notin U_2\\
    \end{cases}
\end{equation}
where $\tilde{\bm{c}}^{2}_{k}$ denote the $k^{\text{th}}$ column of the matrix $\tilde{C}^{T}_{U_2}$ where $\tilde{\bm{c}}^{2}_k$ has zero entries after $k^{\text{th}}$ index since $\tilde{C}^{T}_{U_2}$ is a $(|U_2|\times |U_2|)$ sized lower triangular matrix. Thus, using \refeqn{eqn:Su1_kk} and \ref{eqn:Su2_kk} we have:
\abhinav{See for the case when U1 and U2 have some common intervention. Things might change then!}
\begin{equation}
\begin{aligned}
    \norm{B^{-1}(S_{U_1}-S_{U_2})B^{-T}}_{F}^{2} &\geq \sum_{i\in U_1 \setminus U_2} \Big{[}(\tilde{\bm{c}}^{1}_i)^{T}S{\tilde{\bm{c}}}_i^{1}\Big{]}^{2} + \sum_{j\in U_2\setminus U_1} \Big{[}(\tilde{\bm{c}}^{2}_j)^{T}S{\tilde{\bm{c}}}_j^{2}\Big{]}^{2}\\
    & \geq  \lambda_{min}(S) \Big{[}\sum_{i\in U_1}  \norm{{\tilde{\bm{c}}}_i^{1}}^{2} + \sum_{j\in U_2} \norm{{\tilde{\bm{c}}}_j^{2}}^{2} \Big{]}\\
    &= \lambda_{min}(S) \Big{[} \norm{M_{U_1}C_{U_1}}_F^{2}  + \norm{M_{U_2}C_{U_2}}_{F}^{2} \Big{]}\\
    &\geq \lambda_{min}(S) \Bigg{[} \frac{\norm{C_{U_1}}_{F}^{2}}{\norm{M_{U_1}^{-1}}_{F}^{2}} +  \frac{\norm{C_{U_2}}_{F}^{2}}{\norm{M_{U_2}^{-1}}_{F}^{2}}\Bigg{]} \quad \quad\quad (\because \norm{QR}\geq \frac{\norm{Q^{-1}QR}}{\norm{Q^{-1}}})
\end{aligned}
\end{equation}
\abhinav{Correct above: We don't have full U1 and U2, but the distinct interventions in each}
Next we have:
\begin{equation}
\begin{aligned}
    \norm{M_{U}^{-1}}_{F}^{2} &= \norm{I_{U} + C_{U_1}BE_{U}}_{F}^{2}\\
    &\leq \norm{I_{U}}_{F}^{2}+\norm{C_{U}}^{2}_{F} \norm{B}^{2}_{F}\norm{E_{U}}_{F}^{2}\\
    &= |U|^{2} \Big{(}1+ \norm{C_{U}}_{F}^{2}\norm{B}_{F}^{2}\Big{)}\\
\end{aligned}
\end{equation}
Thus we get:
\begin{equation}
\begin{aligned}
 \norm{S_{U_1}-S_{U_2}}_{F}^{2} \geq \frac{\lambda_{min}(S)}{\norm{B^{-1}}^{4}_{F}}\Bigg{[} \frac{\norm{C_{U_1}}^{2}_{F}}{|U_1|^{2} \Big{(}1+ \norm{C_{U_1}}_{F}^{2}\norm{B}_{F}^{2}\Big{)}}  +  
 \frac{\norm{C_{U_2}}^{2}_{F}}{|U_2|^{2} \Big{(}1+ \norm{C_{U_2}}_{F}^{2}\norm{B}_{F}^{2}\Big{)}}
 \Bigg{]}
\end{aligned}
\end{equation}

\abhinav{Currently adding only selected terms, need to add other terms when we introduce the noise in cov term since these terms will then have a sub}

\end{proof}







==> old_stuff/linear_indep_proof.tex <==
\subsubsection{\textbf{Step2}: Linear independence among $\{S_{i}\}_{i=0}^{n}$}
\label{subsec:step2:independence_known_topo_order}
Next, we will show that the set of \emph{vectorized} covariance matrices of all possible soft atomic interventions along with non-intervened covariance is linearly independent i.e
\begin{equation}
\label{eqn:linear_indep_def}
    \sum_{i\in[n]\cup\{0\}}\alpha_{i}\operatorname{vec}(S_{i})=\bm{0}  \quad \quad \text{iff\space} \alpha_{i}=0, \forall i
\end{equation}
where $n=|\bm{V}|$ is the number of endogenous nodes and $S_{0}\triangleq S$ is the covariance matrix of non-intervened distribution. The following lemma describes the linearity of the ``$\operatorname{vec}$" operator that will help us transform the above equation in the matrix form:
\begin{lemma}[Linearity of ``$\operatorname{vec}$" operator]
\label{lemma:linearity_of_vec_op}
    For a set of matrices $\{M_{j}\}_{j=1}^{n}$ and $n\in\mathbb{N}$, we have $\sum_{j=1}^{n}\operatorname{vec}(M_{j})=\operatorname{vec}(\sum_{j=1}^{n}M_{j})$. 
\end{lemma}
The proof of the above lemma can be found in \refsec{appendix:proof:lemma:linearity_of_vec_op}. Thus using \reflemma{lemma:linearity_of_vec_op} in \refeqn{eqn:linear_indep_def} set $\{\operatorname{vec}(S_{i})\}_{i=0}^{n}$ is linearly independent when:
\begin{equation}
\begin{aligned}
    \sum_{i\in[n]\cup\{0\}} \alpha_{i}S_{i}=\bar{\bm{0}}  \quad \quad \text{iff\space} \alpha_{i}=0, \forall i
\end{aligned}
\end{equation}
where $\bar{\bm{0}}$ is matrix with all zero entries. Given the topological order of the nodes $V_{1}\prec V_{2}\prec \ldots V_{n}$, let the set of nodes $\{V_{1},\ldots V_{r}\}$ be the \emph{\Root} nodes i.e they don't have any parent in the underlying unknown causal graph.
For ease of exposition lets define the sets, $\mathcal{T}_{\text{zero}}\triangleq [n]\cup\{0\}$, $\mathcal{T}_{\text{all}}\triangleq [n]$, $\mathcal{T}_{\text{root}} \triangleq \{1,\ldots,r\}$ where $V_r$ is the last \Root node in the topological order and $\mathcal{T}_{\text{rest}} \triangleq \{{r+1},\ldots,n\}$. 
Now substituting the expression of $S_{i}$ for different intervened distribution from \refeqn{eqn:all_S_i_expression} in the above equation we have to show that:
\begin{equation}
\begin{aligned}
\sum_{i\in\mathcal{T}_{\text{rest}}}&\alpha_{i}\Big{[} \Big{(}\frac{\bm{w}_{i}}{\sqrt{\eta_{i}}}-\sqrt{\eta_{i}}\bm{v}_{i}\Big{)}\Big{(}\frac{\bm{w}_{i}}{\sqrt{\eta_{i}}}-\sqrt{\eta_{i}}\bm{v}_{i}\Big{)}^{T} - \frac{\bm{w}_{i}\bm{w}_{i}^{T}}{\eta_{i}} \Big{]} \\
& +S \Big{[} \sum_{i\in\mathcal{T}_{\text{zero}}}\alpha_{i} \Big{]} - \sum_{i\in\mathcal{T}_{\text{all}}}\Big{[}\alpha_{i}\delta_{i}\bm{v}_{i}\bm{v}_{i}^{T}\Big{]} = \bar{\bm{0}}
\end{aligned}
\end{equation}
iff $\alpha_{i}=0$ for all $i\in[n]\cup\{0\}$. 
Since, $\bm{w}_{i}=BD\bm{u}_{i}=BDB^{T}\bm{c}_{i}=S\bm{c}_{i}$ (from \refeqn{eqn:S_term1_non_root} and \ref{eqn:intervened_B}) and $S^{-1}\bm{v}_{i}=(B^{T})^{-1}D^{-1}B^{-1}\bm{v}_{i}=(B^{T})^{-1}D^{-1}B^{-1}B\bm{e}_{i}=\frac{(I-A)^{T}\bm{e}_{i}}{\sigma_{i}}=\frac{\bm{e}_{i}-\bm{a}_{i}}{\sigma_{i}}$ (since $D^{-1}\bm{e}_{i}=\frac{\bm{e}_{i}}{\sigma_{i}}$ and $B=(I-A)^{-1}$, see \refeqn{eqn:intervened_B} and \ref{eqn:linear_gaussian_sem_def}). Substituting these in the above equation, pre-multiplying and post-multiplying both sides by $S^{-1}=(B^{T})^{-1}D^{-1}B^{-1}$ and rearranging we get:
\begin{equation}
\label{eqn:linear_indep_simplified}
\begin{aligned}
\sum_{i\in\mathcal{T}_{\text{rest}}}\alpha_{i}\Bigg{[}&\Big{(}\frac{\bm{c}_{i}}{\sqrt{\eta_{i}}}-\frac{\sqrt{\eta_{i}}}{\sigma_{i}}(\bm{e}_{i}-\bm{a}_{i})\Big{)}\quad\quad\quad\quad\\
\Big{(}\frac{\bm{c}_{i}}{\sqrt{\eta_{i}}}&-\frac{\sqrt{\eta_{i}}}{\sigma_{i}}(\bm{e}_{i}-\bm{a}_{i})\Big{)}^{T} - \frac{\bm{c}_{i}\bm{c}_{i}^{T}}{\eta_{i}}\Bigg{]}  \quad\quad\quad\quad\\
-\sum_{i\in\mathcal{T}_{\text{all}}}\Bigg{[}&\frac{\alpha_{i}\delta_{i}}{\sigma_{i}^{2}}(\bm{e}_{i}-\bm{a}_{i})(\bm{e}_{i}-\bm{a}_{i})^{T}\Bigg{]} \quad\quad\quad\quad\\
&\quad\quad\quad\quad\quad\quad= S^{-1} \Big{[} -\sum_{i\in\mathcal{T}_{\text{zero}}}\alpha_{i} \Big{]}
\end{aligned}
\end{equation} 
Also notice that the last row of matrix on the LHS of the above equation is only given by $i=n$ and the terms that involve $\bm{e}_{n}$ since $[\bm{c}_{i}]_{n}=0$ and $[\bm{a}_{i}]_{n}=0, \forall i\in \mathcal{T}_{all}$.
Thus for the case when $|\mathcal{T}_{\text{rest}}|\neq0$ the last ($n^{\text{th}}$) row is given by vector:
\begin{equation}
\label{eqn:last_row_non_root}
\begin{aligned}
    \bm{l} &= \frac{-\alpha_{n}}{\sigma_{n}} \Big{[} \Big{(}\bm{c}_{n}-\frac{\eta_{n}}{\sigma_{n}}(\bm{e}_{n}-\bm{a}_{n})\Big{)}+\Big{(}\frac{\delta_{n}}{\sigma_{n}}\Big{)}(\bm{e}_{n}-\bm{a}_{n})\Big{]}\\
    &=\frac{-\alpha_{n}}{\sigma_{n}} \Big{[} \Big{(}1+\frac{\eta_{n}-\delta_{n}}{\sigma_{n}}\Big{)}\bm{a}_{n} - \bm{a}_{n}^{'} - \Big{(} \frac{\eta_{n}-\delta_{n}}{\sigma_{n}}\Big{)} \bm{e}_{n} \Big{]}
\end{aligned}
\end{equation}
Otherwise, when $|\mathcal{T}_{\text{rest}}|=0$ i.e. we only have root nodes in the underlying causal graph, the last ($n^{\text{th}}$) row is given by:
\begin{equation}
\label{eqn:last_row_root}
    \bm{l} = \frac{-\alpha_{n}\delta_{n}}{\sigma_{n}^{2}}[\bm{e}_{n}-\bm{a}_{n}]
\end{equation}
Next, we have two cases based on the value of RHS in the \refeqn{eqn:linear_indep_simplified} above.


\textbf{Case 1:}($\sum_{i\in\mathcal{T}_{\text{zero}}}\alpha_{i}=0$)
Since RHS of \refeqn{eqn:linear_indep_simplified} is zero in this case, we will show that LHS in \refeqn{eqn:linear_indep_simplified} is only zero when all the $\alpha_{i}=0, \forall i\in\mathcal{T}_{\text{all}}$ in the LHS. This will imply that $\alpha_{0}=0$ since we have $\sum_{i\in\mathcal{T}_{\text{zero}}}\alpha_{i}=0$ which will complete our proof showing that $\{\operatorname{vec}(S_{i})\}_{i\in [n]\cup\{0\}}$ are independent. Now, for the case when $|\mathcal{T}_{\text{rest}}|\neq 0$, the $(n,n)^{\text{th}}$ entry of the LHS in \refeqn{eqn:linear_indep_simplified} given by $[\bm{l}]_{n}$ (from \refeqn{eqn:last_row_non_root}) is $\alpha_{n}\big{(}\frac{\eta_{n}-\delta_{n}}{\sigma_{n}^{2}}\big{)}$ since $[\bm{c}_{n}]_{n}=0$ and $[\bm{a}_{n}]_{n}=0$. If $\eta_{n}\neq \delta_{n}$ then this $(n,n)^{\text{th}}$ entry is only zero when $\alpha_{n}=0$ (remember RHS is zero in this case). Otherwise, when $\eta_{n}=\delta_{n}$ then the last row becomes $\frac{-\alpha_{n}}{\sigma_{n}}[\bm{a}_{n}-\bm{a}_{n}^{'}]=\frac{-\alpha_{n}}{\sigma_{n}}\bm{c}_{n}$ and $\bm{c}_{n}\neq\bm{0}$ (from \refassm{assm:effectiveness} for non-root node i.e $n\in\mathcal{T}_{\text{rest}}$). Thus LHS is again zero only when $\alpha_{n}=0$. For the case when $|\mathcal{T}_{\text{rest}}|=0$ i.e when we only have root nodes in the underlying graph, the $(n,n)^{\text{th}}$ entry is given by $[\bm{l}]_{n}=\frac{-\alpha_{n}\delta_{n}}{\sigma_{n}^{2}}$ from \refeqn{eqn:last_row_root}. Since $\delta_{n}\neq 0$ (from \refassm{assm:effectiveness} and $\sigma_{n}\neq 0$ (from the definition linear SEM, see \refsec{sec:prelim}), the LHS is again zero only when $\alpha_{n}=0$. Thus $\alpha_{n}=0$ since the RHS is zero in this case. Next, we can repeat this same procedure iteratively for all LHS rows, i.e.  $i\in\{n-1,\ldots,1\}$, and show that corresponding $\alpha_{i}=0$. This implies that $\alpha_{0}=0$ since $\sum_{i\in[n]\cup\{0\}}\alpha_{i}=0$ and thus the set of vectors $\{\operatorname{vec}(S_{i})\}_{i\in [n]\cup\{0\}}$ are independent. 


\textbf{Case 2:}($\sum_{i\in\mathcal{T}_{\text{zero}}}\alpha_{i}\neq0$)
Since the RHS is not trivially zero this time, we will show that the LHS cannot be equal to RHS if any of the $\alpha_{i}\neq0$. 
The last row of RHS in \refeqn{eqn:linear_indep_simplified} is given by the vector:
\begin{equation}
\label{eqn:last_row_rhs}
    \begin{aligned}
        \bm{r}=\Big{(}-\sum_{i\in \mathcal{T}_{\text{zero}}}\alpha_{i}\Big{)}\frac{(\bm{e}_{n}-\bm{a}_{n})}{\sigma_{n}} 
    \end{aligned}
\end{equation}
since $S^{-1}=(B^{T})^{-1}D^{-1}B^{-1}=(I-A)^{T}D^{-1}(I-A)$ and the last row of $(I-A)^{T}=[0,\ldots,0,1]$ (see definitions of $I,A$ and $D$ in \refsec{sec:prelim}).
\abhinav{Here we use no-product distribution assumption}
From \refassm{assm:no_prod_dist} there is at least one node that is not the the root node in the underlying unknown causal graph. Let that node be the last $V_{n}$. Thus, equating the $(n,n)^{\text{th}}$ entry of the matrix in the LHS and RHS of \refeqn{eqn:linear_indep_simplified} using \refeqn{eqn:last_row_non_root} and \ref{eqn:last_row_rhs} gives us:
\begin{equation}
\label{eqn:case2_n,n_entry}
\begin{aligned}
    \alpha_{n}\frac{(\eta_{n}-\delta_{n})}{\sigma_{n}^{2}} = \frac{1}{\sigma_{n}}\Big{(}-\sum_{i\in \mathcal{T}_{\text{zero}}}\alpha_{i}\Big{)}
\end{aligned}
\end{equation}
where the LHS is given by $[\bm{l}]_{n}$ from \refeqn{eqn:last_row_non_root}. Now looking at $(t,n)^{\text{th}}$ entry on both the side of \refeqn{eqn:linear_indep_simplified} using \refeqn{eqn:last_row_non_root} and \ref{eqn:last_row_rhs}  and substituting the value of $\sum_{i\in \mathcal{T}_{\text{zero}}}\alpha_{i}$ from above equation we get:
\begin{equation}
\begin{aligned}
    \frac{-\alpha_{n}}{\sigma_{n}} &\Big{[} \Big{(}1+\frac{\eta_{n}-\delta_{n}}{\sigma_{n}}\Big{)}[\bm{a}_{n}]_{t} - [\bm{a}_{n}^{'}]_{t} - \Big{(} \frac{\eta_{n}-\delta_{n}}{\sigma_{n}}\Big{)} [\bm{e}_{n}]_{t} \Big{]}\\
    &=\Big{(}-\sum_{i\in \mathcal{T}_{\text{zero}}}\alpha_{i}\Big{)}\frac{[-\bm{a}_{n}]_{t}}{\sigma_{n}}=\alpha_{n}\frac{(\eta_{n}-\delta_{n})}{\sigma_{n}^{2}}[-\bm{a}_{n}]_{t}\\
\end{aligned}
\end{equation}
Rearranging the above equation and substituting $[\bm{e}_{n}]_{t}=0$ for $t\neq n$  we get:
\begin{equation}
\begin{aligned}
    \frac{-\alpha_{n}}{\sigma_{n}} \Big{[} [\bm{a}_{n}]_{t} - [\bm{a}_{n}^{'}]_{t} \Big{]} = 0
\end{aligned}
\end{equation}
From \refassm{assm:effectiveness} $\bm{c}_{n}=\bm{a}_{n}-\bm{a}_{n}^{'}\neq \bm{0}$ for non-root node. Thus $\exists t,\>s.t.\> [\bm{a}_{n}]_{t}-[\bm{a}_{n}^{'}]_{t}\neq 0 \implies $ the above equation is only satisfied when $\alpha_{n}=0$. As a consequence of this, we will show that all the $\alpha_{i}=0$. The rank of matrix on RHS of \refeqn{eqn:linear_indep_simplified} is ``$n$" since $S$ is positive definite and thus and $S^{-1}$ is also positive-definite and thus full-rank matrices. On the left-hand side, we observe that all the matrices corresponding to different $i\in \mathcal{T}_{all}$ have a block structure, where the entries corresponding to index $(m,n)$ are all zero for $m>i$ and $n>i$ for all the $i\in \mathcal{T}_{all}$. Since, $\alpha_{n}=0 \implies$ that the rank of the overall matrix on LHS is less than ``$n$". 

Next, we will show that all the individual matrices on LHS of \refeqn{eqn:linear_indep_simplified} corresponding to different $i\in\mathcal{T}_{all}$ have non-zero entries, and thus the only way \refeqn{eqn:linear_indep_simplified} is satisfied is when all $\alpha_{i}=0, i\in \mathcal{T}_{\text{zero}}$ (since the rank of both sides is different) thereby completing our proof. To show that different matrices corresponding to different ``$i$" are non-zero, it is enough to show that the last row of each of the matrices is non-zero. For a particular index ``$i$" the last row of the corresponding matrix is given by substituting ``$i$" for ``$n$" in \refeqn{eqn:last_row_non_root} and \ref{eqn:last_row_root} based on whether $i\in \mathcal{T}_{\text{rest}}$ or $i\in \mathcal{T}_{\text{root}}$. We can see that the last row for root nodes ($i\in\mathcal{T}_{\text{root}}$) given by \refeqn{eqn:last_row_root} is $ \frac{-\delta_{i}}{\sigma_{i}^{2}}[\bm{e}_{i}-\bm{a}_{i}] \neq \bm{0}$ since $\bm{a}_{i}=0$ and $\delta_{i}\neq0$ (from \refassm{assm:effectiveness}). For non-root nodes i.e $i\in\mathcal{T}_{\text{rest}}$, if $\eta_{i}\neq \delta_{i}$ then the $(i,i)^{\text{th}}$ entry is $\alpha_{i}\big{(}\frac{\eta_{i}-\delta_{i}}{\sigma_{i}^{2}}\big{)}\neq 0$ (\refeqn{eqn:last_row_non_root}). Otherwise, if $\eta_{i}=\delta_{i}$, then the last row vector is $\frac{-\alpha_{i}}{\sigma_{i}}[\bm{a}_{i}-\bm{a}_{i}^{'}]=\frac{-\alpha_{i}}{\sigma_{i}}\bm{c}_{i}$ and $\bm{c}_{i}\neq\bm{0}$ (from \refassm{assm:effectiveness} for non-root node). Thus all the matrices corresponding to different $i\in \mathcal{T}_{\text{all}}$ have non-zero entries. Thus $\alpha_{i}=0$ for all $i\in\mathcal{T}_{\text{all}} \implies \alpha_{0}=0$ since $\sum_{i\in\mathcal{T}_{\text{zero}}}\alpha_{i}=0$ thereby completing our proof for second case.


\subsubsection{\textbf{Step3}: Extending to unknown topological ordering}
\label{subsubsec:step3_unknown_topo_order}

==> old_stuff/old_main_theorem.tex <==
\section{Problem Formulation and Main Theorem}
\label{sec:old_main_theorem}

\abhinav{Describe why mixtures are natural in the real world}
\begin{definition}[Mixture of Soft Atomic Interventions]
\label{def:mixture_of_intervention}
Let $\mathcal{M}=\langle \bm{V},\bm{U},\mathcal{F}\rangle$ be an unknown Gaussian Linear SEM where the distribution of the endogenous variable is given by $\mathbb{P}(\bm{V})$ (see \refsec{sec:prelim}). Let $\mathcal{I}=\{i_1,\ldots,i_K\}$, hereafter referred to as intervention target set, be a set of unknown soft atomic intervention where each $i_k$ generates a new interventional distribution $\mathbb{P}_{i}(\bm{V})$. Then the mixture of soft atomic intervention is defined as:
\begin{equation}
\begin{aligned}
    \mathbb{P}_{mix}(\bm{V}) = \sum_{i_k \in \mathcal{I}} \pi_{i_k} \mathbb{P}_{i_k}(\bm{V})
\end{aligned}
\end{equation}
where $\pi_{i_k}\in \mathbb{R}_{+}$ is a positive scalar s.t. $\sum_{i_k\in\mathcal{I}}\pi_{i_k}=1$, $i_k\in[n]\cup \{0\}$ where $n=|\bm{V}|$ is the number of endogenous variables. We also allow $i_k=0$, which denotes the setting when none of the nodes is intervened and thus $P_{0}(\bm{V})\triangleq\mathbb{P}(\bm{V})$.
\end{definition}


\begin{assumption}[Effectiveness of Soft Intervention]
\label{assm:effectiveness}
     A soft intervention on node $V_{i}$ should change the mechanism in a non-trivial way i.e. $A_{i}\neq A \implies \bm{c}_{i}=\bm{a}_{i}-\bm{a}_{i}^{'}\neq \bm{0}$ for all the $V_{i}$ that are not \emph{\Root} nodes i.e. $\bm{pa}(V_i)\neq \phi$. Also, the noise distribution of any intervened node $V_{i}$ should change i.e. $\bm{\mu}_{i}\neq \bm{\mu}$ \abhinav{Do we need this? Check.} and $D_{i}\neq D \implies \sigma_{i}\neq \sigma_{i}^{'}$ where the intervened noise distribution $\bm{u}_{i}\sim \mathcal{N}(\bm{\mu}_{i}, D_{i})$ and non-intervened noise distribution is given by $\bm{u}\sim \mathcal{N}(\bm{\mu}, D)$. \abhinav{Is it natural to change the noise distribution?}. 
\end{assumption}

% \begin{assumption}[Non collinear Mechanism Change]
% \label{assm:non_collinear_mechanism}
% A soft intervention on node $V_{i}$ should only change the mechanism $\bm{a}_{i}$ to $\bm{a}_{i}^{'}$ s.t. $\bm{a}_{i}\neq \frac{\delta_{i}}{\sigma_{i}}\bm{a}_{i}^{'}$ where $\delta_{i}=\sigma_{i}-\sigma_{i}^{'}$.  \abhinav{Think why this is problematic. Intuitively it will create same covariance i.e. compensate the change in a with sigma'.}
% \end{assumption}


\begin{remark}
The above assumption is sufficient for showing identifiability but not necessary. We conjecture that as long as either the mechanism or the noise distribution changes in the intervened node, the same proof of identifiability should hold (which we have not considered for ease of exposition in this work). We also conjecture that a change in either the mechanism or noise distribution is necessary otherwise we cannot distinguish between the observational (non-intervened) and intervened distribution. This becomes crucial for the nodes that don't have any parents in the underlying unknown causal graph since the mechanism cannot change thus we need to the change noise distribution of those nodes upon intervention to show identifiability. 
\end{remark}


\begin{assumption}[No Product distribution]
\label{assm:no_prod_dist}
\abhinav{Do we need this? Decide after completing proof. If needed then we can mention Bijan's work where they deal with mixture over product distribution.}
\end{assumption}


\begin{theorem}[Disentangling the Mixture]
\label{theorem:main_theorem_disentanglement}
    Given a mixture of soft atomic intervention (\refdef{def:mixture_of_intervention}) over Linear SEM with Gaussian noise (\abhinav{maybe refer this as linear Gaussian additive noise model}) with $\mathcal{I}$ denoting the unknown intervention target set and given \refassm{assm:effectiveness} is satisfied, the following holds:
    \begin{enumerate}
        \item \textbf{Indentifiability}: The parameters of multivariate Gaussian distributions i.e mean $\{\bm{\mu}_{i_{k}}\}_{i_k\in\mathcal{I}}$ and covariance $\{S_{i_k}\}_{i_k\in\mathcal{I}}$ corresponding to each interventional distribution $\{\mathbb{P}_{i_k}(\bm{V})\}_{i_k\in\mathcal{I}}$ present in the mixture is uniquely identifiable \abhinav{along with their mixing proportion $\{\pi_{i_k}\}$?}.
        \item \textbf{Sample Complexity}: \abhinav{TBD after robust kruskal rank proof}
    \end{enumerate}
\end{theorem}

\begin{remark}[Identifiability of Intervention Target set $\mathcal{I}$ and $\mathcal{I}$-MEC]
\abhinav{Here we need to point to the Chandler's, Kartikeyen's (soft) or JCI result on identifiability of unknown intervention from the segregated data.}
    
\end{remark}



==> old_stuff/old_proof_main.tex <==
\section{Proof of Statement 1 of \reftheorem{theorem:main_theorem_disentanglement}}
\label{sec:old_proof_main}

\abhinav{
Proof Outline:
\begin{enumerate}
    \item Show that the set of parameters of the covariance matrix is independent (for a given permutation matrix). What about the $\mu_i$'s? Then show that independent holds for any permutation
    \item Mention and call the black-box result about the Gaussian mixture to identify $S_i$ and conclude identifiability
\end{enumerate}
}

\begin{lemma}[Independence of Covariance matrices]
\label{lemma:independence_covariance}
Let $\mathbb{P}_{i}(\bm{V})$ be the interventional distribution (multivariate Gaussian) generated after soft intervention on node ``$i$" in a linear SEM with Gaussian noise and
let $S_{i}=B_{i}D_{i}B_{i}^{T}$ be the covariance matrix corresponding to  $\mathbb{P}_{i}(\bm{V})$ (see \refsec{sec:prelim}). Then the set of vectors $\mathcal{S}=\{\operatorname{vec}(S_1),\ldots,\operatorname{vec}(S_n)\}\cup\{\operatorname{vec}(S)\}$ are independent where $n=|\bm{V}|$ is the number of endogenous variables, $S$ is the covariance matrix corresponding to $\mathbb{P}(\bm{V})$ and  $\operatorname{vec}$ is an operator that converts a matrix into a vector by concatenating its rows (or columns) as a single columns vector.
\end{lemma}
The proof of above lemma can be found in \refsubsec{subsec:lemma_independence_covariance_proof}.


\subsection{Proof of \reflemma{lemma:independence_covariance}}
\label{subsec:lemma_independence_covariance_proof}
The proof of this lemma proceeds in three steps.
First, given the covariance matrix $S_{0}\triangleq S$ of the non-intervened distribution $\mathbb{P}(V)$, we will show that the covariance matrix ($S_i$) of any intervened distribution $\mathbb{P}_{i}(\bm{V})$ is a rank-3 update on non-intervened covariance matrix $S$. Second, assuming that the correct topological ordering of endogenous variable in the associate unknown causal graph is known \footnote{Given a linear SEM with known adjacency matrix $A$, we can always define a topological order over the endogenous variable denoted as $V_i \prec V_j \Leftrightarrow$ node $V_i$ comes before node $V_j$ in the associated causal graph defined by $A$.}, we show that the set of covariance matrices are independent. Finally, we show that the set of matrices is independent even with unknown topological ordering among endogenous variables.






\subsubsection{\textbf{Step1}: Covariance Matrix Update}
In this and the next subsection, we will assume that the topological ordering of underlying linear SEM is known and without loss of generality, let $V_1\prec V_2\prec\ldots, V_n$ represent the correct topological ordering. Later in \refsec{subsubsec:step3_unknown_topo_order} we will generalize the result to unknown topological ordering. 
Now, from \refeqn{eqn:linear_gaussian_sem_def}, we have $S=BDB^{T}$ where $B=(I-A)^{-1}$ and $A$ is the adjacency matrix of underlying unknown linear SEM. 
Since $V_1\prec,\ldots V_n$ is the correct topological ordering, the adjacency matrix A is a strictly lower triangular, and thus $I-A$ is a lower triangular matrix with all diagonal entries as $1$\abhinav{Do we need to prove this?}. Since $B=(I-A)^{-1}$ and inverse of any lower triangular matrix is also a lower triangular\abhinav{should we cite this result?}, $B$ is also a lower triangular matrix with non-zero diagonal entries. 
Next, we start off by simplifying the expression for the covariance matrix $S_{i}$ for the intervened distribution $\mathbb{P}_{i}(\bm{V})$.  









==> sections/acknowledgement.tex <==
\section*{Acknowledgements}


\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.
